Open Panoramic Segmentation

Panoramic images, capturing a 360{\deg} field of view (FoV), encompass omnidirectional spatial information crucial for scene understanding. However, it is not only costly to obtain training-sufficient dense-annotated panoramas but also application-restricted when training models in a close-vocabulary setting. To tackle this problem, in this work, we define a new task termed Open Panoramic Segmentation (OPS), where models are trained with FoV-restricted pinhole images in the source domain in an open-vocabulary setting while evaluated with FoV-open panoramic images in the target domain, enabling the zero-shot open panoramic semantic segmentation ability of models. Moreover, we propose a model named OOOPS with a Deformable Adapter Network (DAN), which significantly improves zero-shot panoramic semantic segmentation performance. To further enhance the distortion-aware modeling ability from the pinhole source domain, we propose a novel data augmentation method called Random Equirectangular Projection (RERP) which is specifically designed to address object deformations in advance. Surpassing other state-of-the-art open-vocabulary semantic segmentation approaches, a remarkable performance boost on three panoramic datasets, WildPASS, Stanford2D3D, and Matterport3D, proves the effectiveness of our proposed OOOPS model with RERP on the OPS task, especially +2.2% on outdoor WildPASS and +2.4% mIoU on indoor Stanford2D3D. The source code is publicly available at https://junweizheng93.github.io/publications/OPS/OPS.html.

==> tables/rebuttal_RERP_on_other_model.tex <==
\begin{table}[h]
    \centering
    \vskip -3ex
    \caption{mIoU of RERP on other models on WildPASS, Stanford2D3D, and Matterport3D datasets. mIoU is in percentage (\%).}
    \label{tab:rebuttal_RERP_on_other_model}
    \renewcommand{\arraystretch}{0.5}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c l}
        \toprule[1.5pt]
        \textbf{Method} & \textbf{WildPASS} & \textbf{Stanford2D3D} & \textbf{Matterport3D} \\ \midrule\midrule
        SAN (w/ RERP) & 55.6 (+0.9) & 38.5 (+0.5) & 30.5 (+0.4) \\
        \midrule
        CAT-seg (w/ RERP) & 55.7 (+0.8) & 38.6 (+0.5) & 30.2 (+0.7) \\
        \midrule
        OpenSeeD (w/ RERP) & 55.8 (+0.9) & 38.7 (+0.4) & 30.6 (+0.5) \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
\end{table}

==> tables/rebuttal_different_size_RERP.tex <==
\begin{table}[h]
    \centering
    \vskip -2ex
    \caption{mIoU of RERP with adaptive sizes on WildPASS, Stanford2D3D, and Matterport3D datasets. mIoU is in percentage (\%).}
    \label{tab:rebuttal_different_size_RERP}
    \renewcommand{\arraystretch}{0.5}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c l}
        \toprule[1.5pt]
        \textbf{Method} & \textbf{WildPASS} & \textbf{Stanford2D3D} & \textbf{Matterport3D} \\ \midrule\midrule
        RERP & 58.0 & 41.1 & 31.2 \\
        \midrule
        RERP w/ adaptive sizes & \textbf{58.5} & \textbf{41.5} & \textbf{31.6} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    \vskip -4ex
\end{table}

==> tables/rebuttal_importance_of_DAO.tex <==
\begin{table}[h]
    \centering
    \vskip -6ex
    \caption{mIoU w/ and w/o DAO on WildPASS, Stanford2D3D and Matterport3D datasets. mIoU is in percentage (\%).}
    \label{tab:rebuttal_importance_of_DAO}
    \renewcommand{\arraystretch}{0.5}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c l}
        \toprule[1.5pt]
        \textbf{Method} & \textbf{WildPASS} & \textbf{Stanford2D3D} & \textbf{Matterport3D} \\ \midrule\midrule
        OOOPS w/o DAO & 55.6 & 38.5 & 30.5 \\
        \midrule
        OOOPS w/ DAO & \textbf{57.0} & \textbf{39.5} & \textbf{31.1} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    \vskip -2ex
\end{table}

==> tables/rebuttal_rotation.tex <==
\begin{table}[h]
    \centering
    \vskip -3ex
    \caption{mIoU of RERP and simple horizontal rotation on WildPASS, Stanford2D3D, and Matterport3D datasets. mIoU is in percentage (\%).}
    \label{tab:rebuttal_rotation}
    \renewcommand{\arraystretch}{0.5}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c l}
        \toprule[1.5pt]
        \textbf{Method} & \textbf{WildPASS} & \textbf{Stanford2D3D} & \textbf{Matterport3D} \\ \midrule\midrule
        OOOPS w/o RERP & 57.0 & 39.5 & 31.1 \\
        \midrule
        OOOPS w/ Rotation & 57.0 & 39.5 & 31.1 \\
        \midrule
        OOOPS w/ RERP & \textbf{58.0} & \textbf{41.1} & \textbf{31.2} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
    \vskip -2ex
\end{table}
